A tool box for implementing supersymmetric models

We present a framework for performing a comprehensive analysis of a large class of supersymmetric models, including spectrum calculation, dark matter studies and collider phenomenology. To this end, the respective model is defined in an easy and straightforward way using the \Mathematica package SARAH. SARAH then generates model files for CalcHep which can be used with MicrOmegas as well as model files for WHIZARD and OMEGA. In addition, Fortran source code for SPheno is created which facilitates the determination of the particle spectrum using two-loop renormalization group equations and one-loop corrections to the masses. As an additional feature, the generated SPheno code can write out input files suitable for use with HiggsBounds to apply bounds coming from the Higgs searches to the model. Combining all program provides a closed chain from model building to phenomenology.

==> WOcheck.tex <==
\begin{longtable}{|l|cc|cc|c|} 
\hline 
Process & \(\sigma_S\) [fb] & \(\delta_S\) [\%] & \(\sigma_W\) [fb] & \(\delta_W\) [\%] & \(\Delta\) [\%] \\ 
\hline 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow Z Z\) & \(1.227\times 10^{\text{-1}}\) & \(1.19\times 10^{\text{-1}}\) & \(1.227\times 10^{\text{-1}}\) & \(1.2\times 10^{\text{-1}}\) & \(-2.12\times 10^{\text{-2}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow \tilde{\chi}^0_1 \tilde{\chi}^0_1\) & \(2.543\times 10^{\text{-2}}\) & \(6.54\times 10^{\text{-2}}\) & \(2.541\times 10^{\text{-2}}\) & \(6.14\times 10^{\text{-2}}\) & \(7.61\times 10^{\text{-2}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow \tilde{\chi}^0_2 \tilde{\chi}^0_2\) & \(2.217\times 10^{\text{-1}}\) & \(2.67\times 10^{\text{-2}}\) & \(2.217\times 10^{\text{-1}}\) & \(6.32\times 10^{\text{-2}}\) & \(-5.72\times 10^{\text{-3}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow \tilde{\chi}^0_3 \tilde{\chi}^0_3\) & \(1.763\) & \(5.5\times 10^{\text{-2}}\) & \(1.762\) & \(3.49\times 10^{\text{-2}}\) & \(2.56\times 10^{\text{-2}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow \tilde{\chi}^0_4 \tilde{\chi}^0_4\) & \(1.104\) & \(5.14\times 10^{\text{-2}}\) & \(1.106\) & \(4.68\times 10^{\text{-2}}\) & \(-1.85\times 10^{\text{-1}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow h A^0\) & \(3.917\times 10^{\text{-1}}\) & \(4.04\times 10^{\text{-2}}\) & \(3.913\times 10^{\text{-1}}\) & \(4.78\times 10^{\text{-2}}\) & \(9.08\times 10^{\text{-2}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow H A^0\) & \(1.842\) & \(4.64\times 10^{\text{-2}}\) & \(1.841\) & \(4.99\times 10^{\text{-2}}\) & \(3.69\times 10^{\text{-2}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow \tilde{\chi}^+_1 \tilde{\chi}^-_1\) & \(1.069\times 10^{\text{-1}}\) & \(4.76\times 10^{\text{-2}}\) & \(1.068\times 10^{\text{-1}}\) & \(3.94\times 10^{\text{-2}}\) & \(8.89\times 10^{\text{-2}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow \tilde{\chi}^+_2 \tilde{\chi}^-_2\) & \(1.541\) & \(5.22\times 10^{\text{-2}}\) & \(1.54\) & \(5.04\times 10^{\text{-2}}\) & \(1.06\times 10^{\text{-1}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow \tilde{\chi}^0_1 \tilde{\chi}^0_2\) & \(1.505\times 10^{\text{-1}}\) & \(4.46\times 10^{\text{-2}}\) & \(1.506\times 10^{\text{-1}}\) & \(3.69\times 10^{\text{-2}}\) & \(-7.19\times 10^{\text{-2}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow W^- W^+\) & \(1.571\) & \(5.1\times 10^{\text{-2}}\) & \(1.57\) & \(5.47\times 10^{\text{-2}}\) & \(7.34\times 10^{\text{-2}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow d \bar{d}\) & \(6.838\times 10^{\text{-1}}\) & \(2.15\times 10^{\text{-2}}\) & \(6.839\times 10^{\text{-1}}\) & \(5.39\times 10^{\text{-2}}\) & \(-1.13\times 10^{\text{-2}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow t \bar{t}\) & \(1.236\times 10^1\) & \(6.56\times 10^{\text{-2}}\) & \(1.235\times 10^1\) & \(5.13\times 10^{\text{-2}}\) & \(4.62\times 10^{\text{-2}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow b \bar{b}\) & \(7.878\times 10^{\text{-1}}\) & \(2.44\times 10^{\text{-2}}\) & \(7.878\times 10^{\text{-1}}\) & \(2.18\times 10^{\text{-2}}\) & \(-7.2\times 10^{\text{-4}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow \tilde{t}_1 \tilde{t}_1^*\) & \(9.557\) & \(4.66\times 10^{\text{-2}}\) & \(9.561\) & \(4.84\times 10^{\text{-2}}\) & \(-3.94\times 10^{\text{-2}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow \tilde{t}_2 \tilde{t}_2^*\) & \(5.426\times 10^{\text{-1}}\) & \(5.19\times 10^{\text{-2}}\) & \(5.421\times 10^{\text{-1}}\) & \(4.81\times 10^{\text{-2}}\) & \(1.\times 10^{\text{-1}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow \tilde{t}_1 \tilde{t}_2^*\) & \(2.098\) & \(5.43\times 10^{\text{-2}}\) & \(2.097\) & \(5.51\times 10^{\text{-2}}\) & \(6.93\times 10^{\text{-2}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow \tilde{t}_2 \tilde{t}_1^*\) & \(2.097\) & \(4.94\times 10^{\text{-2}}\) & \(2.096\) & \(5.08\times 10^{\text{-2}}\) & \(5.11\times 10^{\text{-2}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow \tilde{d}_1 \tilde{d}_1^*\) & \(1.843\times 10^{\text{-1}}\) & \(5.02\times 10^{\text{-2}}\) & \(1.845\times 10^{\text{-1}}\) & \(5.66\times 10^{\text{-2}}\) & \(-1.29\times 10^{\text{-1}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow \tilde{d}_2 \tilde{d}_2^*\) & \(7.98\times 10^{\text{-1}}\) & \(5.01\times 10^{\text{-2}}\) & \(7.991\times 10^{\text{-1}}\) & \(4.95\times 10^{\text{-2}}\) & \(-1.41\times 10^{\text{-1}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow \tilde{b}_1 \tilde{b}_2^*\) & \(2.059\times 10^{\text{-1}}\) & \(3.75\times 10^{\text{-2}}\) & \(2.059\times 10^{\text{-1}}\) & \(5.04\times 10^{\text{-2}}\) & \(-9.4\times 10^{\text{-3}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow \tilde{b}_2 \tilde{b}_1^*\) & \(2.059\times 10^{\text{-1}}\) & \(4.51\times 10^{\text{-2}}\) & \(2.057\times 10^{\text{-1}}\) & \(4.59\times 10^{\text{-2}}\) & \(7.97\times 10^{\text{-2}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow \nu_e \bar{\nu}_e\) & \(2.209\) & \(6.38\times 10^{\text{-2}}\) & \(2.212\) & \(5.8\times 10^{\text{-2}}\) & \(-1.75\times 10^{\text{-1}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow \nu_\mu \bar{\nu}_\mu\) & \(2.213\) & \(5.83\times 10^{\text{-2}}\) & \(2.213\) & \(5.38\times 10^{\text{-2}}\) & \(1.9\times 10^{\text{-2}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow \tilde{e}_1 \tilde{e}_1^*\) & \(1.073\) & \(5.42\times 10^{\text{-2}}\) & \(1.072\) & \(5.12\times 10^{\text{-2}}\) & \(6.39\times 10^{\text{-2}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow \tilde{e}_2 \tilde{e}_2^*\) & \(2.6\times 10^1\) & \(5.14\times 10^{\text{-2}}\) & \(2.604\times 10^1\) & \(4.49\times 10^{\text{-2}}\) & \(-1.61\times 10^{\text{-1}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow \tilde{\tau}_1 \tilde{\tau}_1^*\) & \(2.145\times 10^1\) & \(5.25\times 10^{\text{-2}}\) & \(2.149\times 10^1\) & \(4.5\times 10^{\text{-2}}\) & \(-1.68\times 10^{\text{-1}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow \tilde{\tau}_2 \tilde{\tau}_2\) & \(4.171\times 10^{\text{-1}}\) & \(4.57\times 10^{\text{-2}}\) & \(4.175\times 10^{\text{-1}}\) & \(4.74\times 10^{\text{-2}}\) & \(-9.82\times 10^{\text{-2}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow \tilde{\tau}_1 \tilde{\tau}_2\) & \(2.642\) & \(5.1\times 10^{\text{-2}}\) & \(2.639\) & \(4.\times 10^{\text{-2}}\) & \(1.03\times 10^{\text{-1}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow \tilde{\tau}_2 \tilde{\tau}_1^*\) & \(2.638\) & \(5.49\times 10^{\text{-2}}\) & \(2.64\) & \(4.53\times 10^{\text{-2}}\) & \(-8.25\times 10^{\text{-2}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow H^- H^+\) & \(1.142\) & \(4.89\times 10^{\text{-2}}\) & \(1.142\) & \(5.33\times 10^{\text{-2}}\) & \(4.09\times 10^{\text{-2}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow h h\) & \(7.944\times 10^{\text{-2}}\) & \(6.73\times 10^{\text{-2}}\) & \(7.963\times 10^{\text{-2}}\) & \(6.51\times 10^{\text{-2}}\) & \(-2.33\times 10^{\text{-1}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow H H\) & \(5.381\times 10^{\text{-2}}\) & \(9.27\times 10^{\text{-2}}\) & \(5.366\times 10^{\text{-2}}\) & \(8.78\times 10^{\text{-2}}\) & \(2.85\times 10^{\text{-1}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow h H\) & \(2.643\times 10^{\text{-1}}\) & \(5.1\times 10^{\text{-2}}\) & \(2.645\times 10^{\text{-1}}\) & \(4.97\times 10^{\text{-2}}\) & \(-8.64\times 10^{\text{-2}}\) \\ 
\(\tilde{\chi}^0_1 \tilde{\chi}^0_1 \rightarrow A^0 A^0\) & \(5.485\times 10^{\text{-2}}\) & \(8.85\times 10^{\text{-2}}\) & \(5.488\times 10^{\text{-2}}\) & \(8.31\times 10^{\text{-2}}\) & \(-5.13\times 10^{\text{-2}}\) \\ 
\(e \bar{e} \rightarrow Z Z\) & \(2.326\) & \(4.93\times 10^{\text{-2}}\) & \(2.326\) & \(5.39\times 10^{\text{-2}}\) & \(1.05\times 10^{\text{-2}}\) \\ 
\(e \bar{e} \rightarrow \gamma \gamma\) & \(1.638\times 10^1\) & \(5.78\times 10^{\text{-2}}\) & \(1.637\times 10^1\) & \(6.04\times 10^{\text{-2}}\) & \(4.12\times 10^{\text{-2}}\) \\ 
\(e \bar{e} \rightarrow \tilde{e}_1 \tilde{e}_1^*\) & \(5.822\) & \(4.9\times 10^{\text{-2}}\) & \(5.82\) & \(5.24\times 10^{\text{-2}}\) & \(2.71\times 10^{\text{-2}}\) \\ 
\(e \bar{e} \rightarrow \tilde{e}_2 \tilde{e}_2^*\) & \(4.964\) & \(5.9\times 10^{\text{-2}}\) & \(4.96\) & \(4.8\times 10^{\text{-2}}\) & \(6.55\times 10^{\text{-2}}\) \\ 
\(e \bar{e} \rightarrow \tilde{\chi}^0_1 \tilde{\chi}^0_1\) & \(1.144\times 10^1\) & \(6.52\times 10^{\text{-2}}\) & \(1.143\times 10^1\) & \(1.09\times 10^{\text{-2}}\) & \(4.81\times 10^{\text{-2}}\) \\ 
\(e \bar{e} \rightarrow \tilde{\chi}^0_2 \tilde{\chi}^0_2\) & \(8.506\) & \(6.56\times 10^{\text{-2}}\) & \(8.499\) & \(4.38\times 10^{\text{-2}}\) & \(7.95\times 10^{\text{-2}}\) \\ 
\(e \bar{e} \rightarrow \tilde{\chi}^0_3 \tilde{\chi}^0_3\) & \(1.489\times 10^{\text{-3}}\) & \(5.28\times 10^{\text{-2}}\) & \(1.488\times 10^{\text{-3}}\) & \(3.44\times 10^{\text{-2}}\) & \(7.08\times 10^{\text{-2}}\) \\ 
\(e \bar{e} \rightarrow \tilde{\chi}^0_4 \tilde{\chi}^0_4\) & \(4.229\times 10^{\text{-2}}\) & \(5.50\times 10^{\text{-2}}\) & \(4.238\times 10^{\text{-2}}\) & \(6.43\times 10^{\text{-2}}\) & \(-2.02\times 10^{\text{-1}}\) \\ 
\(e \bar{e} \rightarrow h A^0\) & \(1.932\times 10^{\text{-4}}\) & \(4.68\times 10^{\text{-2}}\) & \(1.931\times 10^{\text{-4}}\) & \(1.00\times 10^{\text{-2}}\) & \(8.58\times 10^{\text{-3}}\) \\ 
\(e \bar{e} \rightarrow H A^0\) & \(1.35\) & \(5.4\times 10^{\text{-2}}\) & \(1.351\) & \(7.94\times 10^{\text{-3}}\) & \(-9.42\times 10^{\text{-2}}\) \\ 
\(e \bar{e} \rightarrow \tilde{\chi}^+_1 \tilde{\chi}^-_1\) & \(1.658\times 10^1\) & \(5.82\times 10^{\text{-2}}\) & \(1.658\times 10^1\) & \(5.21\times 10^{\text{-2}}\) & \(1.7\times 10^{\text{-2}}\) \\ 
\(e \bar{e} \rightarrow \tilde{\chi}^+_2 \tilde{\chi}^-_2\) & \(9.636\) & \(4.87\times 10^{\text{-2}}\) & \(9.612\) & \(4.94\times 10^{\text{-2}}\) & \(2.44\times 10^{\text{-1}}\) \\ 
\(e \bar{e} \rightarrow \tilde{\chi}^0_1 \tilde{\chi}^0_2\) & \(4.362\) & \(5.23\times 10^{\text{-2}}\) & \(4.359\) & \(5.47\times 10^{\text{-2}}\) & \(5.51\times 10^{\text{-2}}\) \\ 
\(e \bar{e} \rightarrow W^- W^+\) & \(2.658\times 10^1\) & \(5.69\times 10^{\text{-2}}\) & \(2.659\times 10^1\) & \(5.58\times 10^{\text{-2}}\) & \(-1.81\times 10^{\text{-2}}\) \\ 
\(e \bar{e} \rightarrow d \bar{d}\) & \(7.546\) & \(3.62\times 10^{\text{-2}}\) & \(7.555\) & \(2.52\times 10^{\text{-2}}\) & \(-1.16\times 10^{\text{-1}}\) \\ 
\(e \bar{e} \rightarrow t \bar{t}\) & \(1.428\times 10^1\) & \(1.6\times 10^{\text{-2}}\) & \(1.428\times 10^1\) & \(1.6\times 10^{\text{-2}}\) & \(-5.32\times 10^{\text{-2}}\) \\ 
\(e \bar{e} \rightarrow b \bar{b}\) & \(7.557\) & \(4.18\times 10^{\text{-2}}\) & \(7.564\) & \(1.82\times 10^{\text{-2}}\) & \(-1.\times 10^{\text{-1}}\) \\ 
\(e \bar{e} \rightarrow \tilde{t}_1 \tilde{t}_1^*\) & \(3.693\) & \(7.9\times 10^{\text{-3}}\) & \(3.694\) & \(7.97\times 10^{\text{-3}}\) & \(-3.42\times 10^{\text{-2}}\) \\ 
\(e \bar{e} \rightarrow \tilde{t}_2 \tilde{t}_2^*\) & \(3.091\) & \(9.08\times 10^{\text{-3}}\) & \(3.091\) & \(6.61\times 10^{\text{-3}}\) & \(1.02\times 10^{\text{-2}}\) \\ 
\(e \bar{e} \rightarrow \tilde{t}_1 \tilde{t}_2^*\) & \(7.907\times 10^{\text{-1}}\) & \(7.81\times 10^{\text{-3}}\) & \(7.905\times 10^{\text{-1}}\) & \(7.07\times 10^{\text{-3}}\) & \(2.42\times 10^{\text{-2}}\) \\ 
\(e \bar{e} \rightarrow \tilde{t}_2 \tilde{t}_1^*\) & \(7.906\times 10^{\text{-1}}\) & \(6.69\times 10^{\text{-3}}\) & \(7.905\times 10^{\text{-1}}\) & \(8.49\times 10^{\text{-3}}\) & \(1.2\times 10^{\text{-2}}\) \\ 
\(e \bar{e} \rightarrow \tilde{d}_1 \tilde{d}_1^*\) & \(3.087\) & \(6.29\times 10^{\text{-3}}\) & \(3.087\) & \(1.47\times 10^{\text{-2}}\) & \(-1.51\times 10^{\text{-3}}\) \\ 
\(e \bar{e} \rightarrow \tilde{d}_2 \tilde{d}_2^*\) & \(6.913\times 10^{\text{-1}}\) & \(1.\times 10^{\text{-2}}\) & \(6.912\times 10^{\text{-1}}\) & \(8.34\times 10^{\text{-3}}\) & \(8.73\times 10^{\text{-3}}\) \\ 
\(e \bar{e} \rightarrow \tilde{b}_1 \tilde{b}_2^*\) & \(3.483\times 10^{\text{-1}}\) & \(9.12\times 10^{\text{-3}}\) & \(3.484\times 10^{\text{-1}}\) & \(6.08\times 10^{\text{-3}}\) & \(-2.67\times 10^{\text{-2}}\) \\ 
\(e \bar{e} \rightarrow \tilde{b}_2 \tilde{b}_1^*\) & \(3.484\times 10^{\text{-1}}\) & \(6.59\times 10^{\text{-3}}\) & \(3.484\times 10^{\text{-1}}\) & \(8.2\times 10^{\text{-3}}\) & \(1.16\times 10^{\text{-4}}\) \\ 
\(e \bar{e} \rightarrow \nu_\mu \bar{\nu}_\mu\) & \(2.041\) & \(5.09\times 10^{\text{-3}}\) & \(2.039\) & \(1.86\times 10^{\text{-2}}\) & \(7.4\times 10^{\text{-2}}\) \\ 
\(e \bar{e} \rightarrow \tilde{\tau}_1 \tilde{\tau}_1^*\) & \(3.382\) & \(1.03\times 10^{\text{-2}}\) & \(3.382\) & \(5.6\times 10^{\text{-3}}\) & \(1.14\times 10^{\text{-2}}\) \\ 
\(e \bar{e} \rightarrow \tilde{\tau}_2 \tilde{\tau}_2\) & \(3.815\) & \(8.34\times 10^{\text{-3}}\) & \(3.816\) & \(8.21\times 10^{\text{-3}}\) & \(-2.25\times 10^{\text{-3}}\) \\ 
\(e \bar{e} \rightarrow \tilde{\tau}_1 \tilde{\tau}_2\) & \(1.561\times 10^{\text{-1}}\) & \(9.63\times 10^{\text{-3}}\) & \(1.561\times 10^{\text{-1}}\) & \(7.14\times 10^{\text{-3}}\) & \(-5.58\times 10^{\text{-3}}\) \\ 
\(e \bar{e} \rightarrow \tilde{\tau}_2 \tilde{\tau}_1^*\) & \(1.56\times 10^{\text{-1}}\) & \(8.24\times 10^{\text{-3}}\) & \(1.56\times 10^{\text{-1}}\) & \(8.52\times 10^{\text{-3}}\) & \(1.3\times 10^{\text{-2}}\) \\ 
\(e \bar{e} \rightarrow \gamma Z\) & \(1.206\times 10^1\) & \(6.05\times 10^{\text{-2}}\) & \(1.205\times 10^1\) & \(6.07\times 10^{\text{-2}}\) & \(8.77\times 10^{\text{-2}}\) \\ 
\(e \bar{e} \rightarrow H^- H^+\) & \(3.147\) & \(3.66\times 10^{\text{-2}}\) & \(3.148\) & \(7.18\times 10^{\text{-3}}\) & \(-4.64\times 10^{\text{-2}}\) \\ 
\(\tau \bar{\tau} \rightarrow Z Z\) & \(2.323\) & \(5.25\times 10^{\text{-2}}\) & \(2.326\) & \(5.95\times 10^{\text{-2}}\) & \(-1.02\times 10^{\text{-1}}\) \\ 
\(\tau \bar{\tau} \rightarrow \gamma \gamma\) & \(1.636\times 10^1\) & \(5.28\times 10^{\text{-2}}\) & \(1.639\times 10^1\) & \(6.19\times 10^{\text{-2}}\) & \(-2.16\times 10^{\text{-1}}\) \\ 
\(\tau \bar{\tau} \rightarrow \tilde{\chi}^0_1 \tilde{\chi}^0_1\) & \(1.148\times 10^1\) & \(6.75\times 10^{\text{-2}}\) & \(1.147\times 10^1\) & \(6.17\times 10^{\text{-2}}\) & \(2.72\times 10^{\text{-3}}\) \\ 
\(\tau \bar{\tau} \rightarrow \tilde{\chi}^0_2 \tilde{\chi}^0_2\) & \(8.575\) & \(6.2\times 10^{\text{-2}}\) & \(8.575\) & \(3.4\times 10^{\text{-2}}\) & \(-4.36\times 10^{\text{-3}}\) \\ 
\(\tau \bar{\tau} \rightarrow \tilde{\chi}^0_3 \tilde{\chi}^0_3\) & \(1.806\times 10^{\text{-2}}\) & \(5.86\times 10^{\text{-2}}\) & \(1.807\times 10^{\text{-2}}\) & \(5.12\times 10^{\text{-2}}\) & \(-3.57\times 10^{\text{-2}}\) \\ 
\(\tau \bar{\tau} \rightarrow \tilde{\chi}^0_4 \tilde{\chi}^0_4\) & \(8.167\times 10^{\text{-2}}\) & \(5.04\times 10^{\text{-2}}\) & \(8.169\times 10^{\text{-2}}\) & \(6.13\times 10^{\text{-2}}\) & \(-3.52\times 10^{\text{-2}}\) \\ 
\(\tau \bar{\tau} \rightarrow h A^0\) & \(6.966\times 10^{\text{-4}}\) & \(5.32\times 10^{\text{-2}}\) & \(6.975\times 10^{\text{-4}}\) & \(5.21\times 10^{\text{-2}}\) & \(-1.21\times 10^{\text{-1}}\) \\ 
\(\tau \bar{\tau} \rightarrow H A^0\) & \(9.219\times 10^{\text{-1}}\) & \(5.11\times 10^{\text{-2}}\) & \(9.216\times 10^{\text{-1}}\) & \(4.26\times 10^{\text{-2}}\) & \(3.03\times 10^{\text{-2}}\) \\ 
\(\tau \bar{\tau} \rightarrow \tilde{\chi}^+_1 \tilde{\chi}^-_1\) & \(1.661\times 10^1\) & \(5.28\times 10^{\text{-2}}\) & \(1.658\times 10^1\) & \(5.12\times 10^{\text{-2}}\) & \(2.07\times 10^{\text{-1}}\) \\ 
\(\tau \bar{\tau} \rightarrow \tilde{\chi}^+_2 \tilde{\chi}^-_2\) & \(9.421\) & \(4.73\times 10^{\text{-2}}\) & \(9.409\) & \(4.72\times 10^{\text{-2}}\) & \(1.27\times 10^{\text{-1}}\) \\ 
\(\tau \bar{\tau} \rightarrow \tilde{\chi}^0_1 \tilde{\chi}^0_2\) & \(4.329\) & \(5.61\times 10^{\text{-2}}\) & \(4.329\) & \(5.95\times 10^{\text{-2}}\) & \(2.05\times 10^{\text{-3}}\) \\ 
\(\tau \bar{\tau} \rightarrow W^- W^+\) & \(2.658\times 10^1\) & \(5.36\times 10^{\text{-2}}\) & \(2.661\times 10^1\) & \(5.71\times 10^{\text{-2}}\) & \(-9.94\times 10^{\text{-2}}\) \\ 
\(\tau \bar{\tau} \rightarrow d \bar{d}\) & \(7.555\) & \(5.11\times 10^{\text{-2}}\) & \(7.56\) & \(2.47\times 10^{\text{-2}}\) & \(-7.55\times 10^{\text{-2}}\) \\ 
\(\tau \bar{\tau} \rightarrow t \bar{t}\) & \(1.428\times 10^1\) & \(1.46\times 10^{\text{-2}}\) & \(1.428\times 10^1\) & \(1.61\times 10^{\text{-2}}\) & \(-1.81\times 10^{\text{-2}}\) \\ 
\(\tau \bar{\tau} \rightarrow b \bar{b}\) & \(8.383\) & \(5.09\times 10^{\text{-2}}\) & \(8.381\) & \(3.93\times 10^{\text{-2}}\) & \(2.09\times 10^{\text{-2}}\) \\ 
\(\tau \bar{\tau} \rightarrow \tilde{t}_1 \tilde{t}_1^*\) & \(3.803\) & \(6.31\times 10^{\text{-3}}\) & \(3.804\) & \(8.3\times 10^{\text{-3}}\) & \(-1.26\times 10^{\text{-2}}\) \\ 
\(\tau \bar{\tau} \rightarrow \tilde{t}_2 \tilde{t}_2^*\) & \(3.187\) & \(7.98\times 10^{\text{-3}}\) & \(3.187\) & \(9.49\times 10^{\text{-3}}\) & \(-3.73\times 10^{\text{-3}}\) \\ 
\(\tau \bar{\tau} \rightarrow \tilde{t}_1 \tilde{t}_2^*\) & \(9.572\times 10^{\text{-1}}\) & \(7.54\times 10^{\text{-3}}\) & \(9.573\times 10^{\text{-1}}\) & \(7.16\times 10^{\text{-3}}\) & \(-2.47\times 10^{\text{-3}}\) \\ 
\(\tau \bar{\tau} \rightarrow \tilde{t}_2 \tilde{t}_1^*\) & \(9.57\times 10^{\text{-1}}\) & \(8.39\times 10^{\text{-3}}\) & \(9.572\times 10^{\text{-1}}\) & \(7.43\times 10^{\text{-3}}\) & \(-2.12\times 10^{\text{-2}}\) \\ 
\(\tau \bar{\tau} \rightarrow \tilde{d}_1 \tilde{d}_1^*\) & \(3.087\) & \(7.9\times 10^{\text{-3}}\) & \(3.087\) & \(9.86\times 10^{\text{-3}}\) & \(2.05\times 10^{\text{-2}}\) \\ 
\(\tau \bar{\tau} \rightarrow \tilde{d}_2 \tilde{d}_2^*\) & \(6.912\times 10^{\text{-1}}\) & \(7.66\times 10^{\text{-3}}\) & \(6.912\times 10^{\text{-1}}\) & \(8.46\times 10^{\text{-3}}\) & \(1.29\times 10^{\text{-3}}\) \\ 
\(\tau \bar{\tau} \rightarrow \tilde{b}_1 \tilde{b}_2^*\) & \(3.484\times 10^{\text{-1}}\) & \(7.54\times 10^{\text{-3}}\) & \(3.483\times 10^{\text{-1}}\) & \(7.27\times 10^{\text{-3}}\) & \(2.01\times 10^{\text{-2}}\) \\ 
\(\tau \bar{\tau} \rightarrow \tilde{b}_2 \tilde{b}_1^*\) & \(3.484\times 10^{\text{-1}}\) & \(7.28\times 10^{\text{-3}}\) & \(3.484\times 10^{\text{-1}}\) & \(7.25\times 10^{\text{-3}}\) & \(-9.98\times 10^{\text{-3}}\) \\ 
\(\tau \bar{\tau} \rightarrow \nu_e \bar{\nu}_e\) & \(2.038\) & \(2.89\times 10^{\text{-2}}\) & \(2.039\) & \(1.78\times 10^{\text{-2}}\) & \(-6.52\times 10^{\text{-2}}\) \\ 
\(\tau \bar{\tau} \rightarrow \nu_\mu \bar{\nu}_\mu\) & \(2.038\) & \(1.98\times 10^{\text{-2}}\) & \(2.038\) & \(1.87\times 10^{\text{-2}}\) & \(1.83\times 10^{\text{-3}}\) \\ 
\(\tau \bar{\tau} \rightarrow \tilde{e}_1 \tilde{e}_1^*\) & \(4.052\) & \(8.94\times 10^{\text{-3}}\) & \(4.051\) & \(7.61\times 10^{\text{-3}}\) & \(4.\times 10^{\text{-3}}\) \\ 
\(\tau \bar{\tau} \rightarrow \tilde{e}_2 \tilde{e}_2^*\) & \(3.446\) & \(8.12\times 10^{\text{-3}}\) & \(3.446\) & \(7.45\times 10^{\text{-3}}\) & \(-1.36\times 10^{\text{-2}}\) \\ 
\(\tau \bar{\tau} \rightarrow \tilde{\tau}_1 \tilde{\tau}_1^*\) & \(3.452\) & \(5.31\times 10^{\text{-2}}\) & \(3.454\) & \(4.85\times 10^{\text{-2}}\) & \(-5.53\times 10^{\text{-2}}\) \\ 
\(\tau \bar{\tau} \rightarrow \tilde{\tau}_2 \tilde{\tau}_2\) & \(4.13\) & \(5.76\times 10^{\text{-2}}\) & \(4.136\) & \(4.72\times 10^{\text{-2}}\) & \(-1.37\times 10^{\text{-1}}\) \\ 
\(\tau \bar{\tau} \rightarrow \tilde{\tau}_1 \tilde{\tau}_2\) & \(1.426\) & \(4.65\times 10^{\text{-2}}\) & \(1.425\) & \(4.73\times 10^{\text{-2}}\) & \(1.19\times 10^{\text{-1}}\) \\ 
\(\tau \bar{\tau} \rightarrow \tilde{\tau}_2 \tilde{\tau}_1^*\) & \(1.424\) & \(4.68\times 10^{\text{-2}}\) & \(1.425\) & \(4.72\times 10^{\text{-2}}\) & \(-6.04\times 10^{\text{-2}}\) \\ 
\(\tau \bar{\tau} \rightarrow \gamma Z\) & \(1.206\times 10^1\) & \(5.82\times 10^{\text{-2}}\) & \(1.206\times 10^1\) & \(5.04\times 10^{\text{-2}}\) & \(-2.91\times 10^{\text{-2}}\) \\ 
\(\tau \bar{\tau} \rightarrow H^- H^+\) & \(2.963\) & \(4.32\times 10^{\text{-2}}\) & \(2.964\) & \(3.8\times 10^{\text{-2}}\) & \(-3.81\times 10^{\text{-2}}\) \\ 
\(\tau \bar{\tau} \rightarrow h h\) & \(3.539\times 10^{\text{-5}}\) & \(6.28\times 10^{\text{-2}}\) & \(3.538\times 10^{\text{-5}}\) & \(4.06\times 10^{\text{-2}}\) & \(3.31\times 10^{\text{-2}}\) \\ 
\(\tau \bar{\tau} \rightarrow H H\) & \(1.315\times 10^{\text{-3}}\) & \(8.67\times 10^{\text{-2}}\) & \(1.318\times 10^{\text{-3}}\) & \(8.42\times 10^{\text{-2}}\) & \(-2.23\times 10^{\text{-1}}\) \\ 
\(\tau \bar{\tau} \rightarrow h H\) & \(5.753\times 10^{\text{-4}}\) & \(5.03\times 10^{\text{-2}}\) & \(5.758\times 10^{\text{-4}}\) & \(4.89\times 10^{\text{-2}}\) & \(-9.88\times 10^{\text{-2}}\) \\ 
\(\tau \bar{\tau} \rightarrow A^0 A^0\) & \(1.257\times 10^{\text{-3}}\) & \(9.00\times 10^{\text{-2}}\) & \(1.257\times 10^{\text{-3}}\) & \(8.87\times 10^{\text{-2}}\) & \(7.02\times 10^{\text{-2}}\) \\ 
\(d \bar{d} \rightarrow Z Z\) & \(3.044\) & \(5.59\times 10^{\text{-2}}\) & \(3.043\) & \(6.28\times 10^{\text{-2}}\) & \(1.52\times 10^{\text{-2}}\) \\ 
\(d \bar{d} \rightarrow \gamma \gamma\) & \(6.739\times 10^{\text{-2}}\) & \(6.58\times 10^{\text{-2}}\) & \(6.741\times 10^{\text{-2}}\) & \(7.81\times 10^{\text{-2}}\) & \(-1.98\times 10^{\text{-2}}\) \\ 
\(d \bar{d} \rightarrow \tilde{\chi}^0_1 \tilde{\chi}^0_1\) & \(3.763\times 10^{\text{-2}}\) & \(3.78\times 10^{\text{-2}}\) & \(3.768\times 10^{\text{-2}}\) & \(5.78\times 10^{\text{-2}}\) & \(-1.13\times 10^{\text{-1}}\) \\ 
\(d \bar{d} \rightarrow \tilde{\chi}^0_2 \tilde{\chi}^0_2\) & \(1.548\) & \(3.4\times 10^{\text{-2}}\) & \(1.546\) & \(5.13\times 10^{\text{-2}}\) & \(1.43\times 10^{\text{-1}}\) \\ 
\(d \bar{d} \rightarrow \tilde{\chi}^0_3 \tilde{\chi}^0_3\) & \(9.433\times 10^{\text{-4}}\) & \(5.42\times 10^{\text{-2}}\) & \(9.404\times 10^{\text{-4}}\) & \(5.80\times 10^{\text{-2}}\) & \(3.11\times 10^{\text{-1}}\) \\ 
\(d \bar{d} \rightarrow \tilde{\chi}^0_4 \tilde{\chi}^0_4\) & \(2.998\times 10^{\text{-2}}\) & \(6.14\times 10^{\text{-2}}\) & \(2.996\times 10^{\text{-2}}\) & \(5.44\times 10^{\text{-2}}\) & \(6.82\times 10^{\text{-2}}\) \\ 
\(d \bar{d} \rightarrow h A^0\) & \(9.525\times 10^{\text{-5}}\) & \(4.51\times 10^{\text{-2}}\) & \(9.512\times 10^{\text{-5}}\) & \(8.14\times 10^{\text{-3}}\) & \(1.31\times 10^{\text{-1}}\) \\ 
\(d \bar{d} \rightarrow H A^0\) & \(6.646\times 10^{\text{-1}}\) & \(5.58\times 10^{\text{-2}}\) & \(6.653\times 10^{\text{-1}}\) & \(8.32\times 10^{\text{-3}}\) & \(-1.13\times 10^{\text{-1}}\) \\ 
\(d \bar{d} \rightarrow \tilde{\chi}^+_1 \tilde{\chi}^-_1\) & \(4.137\) & \(5.2\times 10^{\text{-2}}\) & \(4.144\) & \(5.12\times 10^{\text{-2}}\) & \(-1.52\times 10^{\text{-1}}\) \\ 
\(d \bar{d} \rightarrow \tilde{\chi}^+_2 \tilde{\chi}^-_2\) & \(1.532\) & \(4.74\times 10^{\text{-2}}\) & \(1.53\) & \(4.88\times 10^{\text{-2}}\) & \(9.91\times 10^{\text{-2}}\) \\ 
\(d \bar{d} \rightarrow \tilde{\chi}^0_1 \tilde{\chi}^0_2\) & \(1.734\times 10^{\text{-1}}\) & \(5.02\times 10^{\text{-2}}\) & \(1.733\times 10^{\text{-1}}\) & \(5.54\times 10^{\text{-2}}\) & \(4.12\times 10^{\text{-2}}\) \\ 
\(d \bar{d} \rightarrow W^- W^+\) & \(8.037\) & \(5.28\times 10^{\text{-2}}\) & \(8.048\) & \(5.24\times 10^{\text{-2}}\) & \(-1.43\times 10^{\text{-1}}\) \\ 
\(d \bar{d} \rightarrow d \bar{d}\) & \(5.623\times 10^3\) & \(6.45\times 10^{\text{-2}}\) & \(5.632\times 10^3\) & \(4.23\times 10^{\text{-2}}\) & \(-1.63\times 10^{\text{-1}}\) \\ 
\(d \bar{d} \rightarrow t \bar{t}\) & \(4.224\times 10^2\) & \(9.75\times 10^{\text{-3}}\) & \(4.222\times 10^2\) & \(9.43\times 10^{\text{-3}}\) & \(3.4\times 10^{\text{-2}}\) \\ 
\(d \bar{d} \rightarrow b \bar{b}\) & \(4.177\times 10^2\) & \(4.55\times 10^{\text{-2}}\) & \(4.177\times 10^2\) & \(2.72\times 10^{\text{-2}}\) & \(1.32\times 10^{\text{-3}}\) \\ 
\(d \bar{d} \rightarrow \tilde{t}_1 \tilde{t}_1^*\) & \(1.493\times 10^2\) & \(8.46\times 10^{\text{-3}}\) & \(1.493\times 10^2\) & \(8.12\times 10^{\text{-3}}\) & \(-1.42\times 10^{\text{-2}}\) \\ 
\(d \bar{d} \rightarrow \tilde{t}_2 \tilde{t}_2^*\) & \(9.921\times 10^1\) & \(8.41\times 10^{\text{-3}}\) & \(9.922\times 10^1\) & \(7.97\times 10^{\text{-3}}\) & \(-8.73\times 10^{\text{-3}}\) \\ 
\(d \bar{d} \rightarrow \tilde{t}_1 \tilde{t}_2^*\) & \(3.893\times 10^{\text{-1}}\) & \(6.69\times 10^{\text{-3}}\) & \(3.893\times 10^{\text{-1}}\) & \(8.03\times 10^{\text{-3}}\) & \(1.3\times 10^{\text{-2}}\) \\ 
\(d \bar{d} \rightarrow \tilde{t}_2 \tilde{t}_1^*\) & \(3.894\times 10^{\text{-1}}\) & \(8.13\times 10^{\text{-3}}\) & \(3.892\times 10^{\text{-1}}\) & \(8.42\times 10^{\text{-3}}\) & \(3.89\times 10^{\text{-2}}\) \\ 
\(d \bar{d} \rightarrow \tilde{d}_1 \tilde{d}_1^*\) & \(3.288\times 10^2\) & \(6.04\times 10^{\text{-2}}\) & \(3.286\times 10^2\) & \(6.16\times 10^{\text{-2}}\) & \(6.86\times 10^{\text{-2}}\) \\ 
\(d \bar{d} \rightarrow \tilde{d}_2 \tilde{d}_2^*\) & \(3.975\times 10^2\) & \(4.72\times 10^{\text{-2}}\) & \(3.973\times 10^2\) & \(3.86\times 10^{\text{-2}}\) & \(3.96\times 10^{\text{-2}}\) \\ 
\(d \bar{d} \rightarrow \tilde{b}_1 \tilde{b}_2^*\) & \(1.715\times 10^{\text{-1}}\) & \(1.48\times 10^{\text{-2}}\) & \(1.715\times 10^{\text{-1}}\) & \(6.82\times 10^{\text{-3}}\) & \(-3.92\times 10^{\text{-2}}\) \\ 
\(d \bar{d} \rightarrow \tilde{b}_2 \tilde{b}_1^*\) & \(1.715\times 10^{\text{-1}}\) & \(8.57\times 10^{\text{-3}}\) & \(1.715\times 10^{\text{-1}}\) & \(1.46\times 10^{\text{-2}}\) & \(1.5\times 10^{\text{-2}}\) \\ 
\(d \bar{d} \rightarrow \nu_e \bar{\nu}_e\) & \(1.003\) & \(3.63\times 10^{\text{-2}}\) & \(1.003\) & \(2.41\times 10^{\text{-2}}\) & \(-7.7\times 10^{\text{-2}}\) \\ 
\(d \bar{d} \rightarrow \nu_\mu \bar{\nu}_\mu\) & \(1.003\) & \(2.44\times 10^{\text{-2}}\) & \(1.004\) & \(1.97\times 10^{\text{-2}}\) & \(-8.11\times 10^{\text{-2}}\) \\ 
\(d \bar{d} \rightarrow \tilde{e}_1 \tilde{e}_1^*\) & \(5.842\times 10^{\text{-1}}\) & \(7.11\times 10^{\text{-3}}\) & \(5.843\times 10^{\text{-1}}\) & \(7.58\times 10^{\text{-3}}\) & \(-1.02\times 10^{\text{-2}}\) \\ 
\(d \bar{d} \rightarrow \tilde{e}_2 \tilde{e}_2^*\) & \(1.28\times 10^{\text{-1}}\) & \(8.69\times 10^{\text{-3}}\) & \(1.28\times 10^{\text{-1}}\) & \(7.45\times 10^{\text{-3}}\) & \(-3.33\times 10^{\text{-3}}\) \\ 
\(d \bar{d} \rightarrow \tilde{\tau}_1 \tilde{\tau}_1^*\) & \(9.771\times 10^{\text{-2}}\) & \(8.29\times 10^{\text{-3}}\) & \(9.771\times 10^{\text{-2}}\) & \(8.78\times 10^{\text{-3}}\) & \(4.69\times 10^{\text{-3}}\) \\ 
\(d \bar{d} \rightarrow \tilde{\tau}_2 \tilde{\tau}_2\) & \(4.618\times 10^{\text{-1}}\) & \(7.19\times 10^{\text{-3}}\) & \(4.617\times 10^{\text{-1}}\) & \(6.64\times 10^{\text{-3}}\) & \(2.34\times 10^{\text{-2}}\) \\ 
\(d \bar{d} \rightarrow \tilde{\tau}_1 \tilde{\tau}_2\) & \(7.683\times 10^{\text{-2}}\) & \(8.29\times 10^{\text{-3}}\) & \(7.683\times 10^{\text{-2}}\) & \(8.51\times 10^{\text{-3}}\) & \(-4.12\times 10^{\text{-3}}\) \\ 
\(d \bar{d} \rightarrow \tilde{\tau}_2 \tilde{\tau}_1^*\) & \(7.680\times 10^{\text{-2}}\) & \(1.52\times 10^{\text{-2}}\) & \(7.681\times 10^{\text{-2}}\) & \(1.49\times 10^{\text{-2}}\) & \(-1.89\times 10^{\text{-2}}\) \\ 
\(d \bar{d} \rightarrow \gamma Z\) & \(6.592\times 10^{\text{-1}}\) & \(7.4\times 10^{\text{-2}}\) & \(6.59\times 10^{\text{-1}}\) & \(5.59\times 10^{\text{-2}}\) & \(3.73\times 10^{\text{-2}}\) \\ 
\(d \bar{d} \rightarrow H^- H^+\) & \(4.544\times 10^{\text{-1}}\) & \(4.37\times 10^{\text{-2}}\) & \(4.54\times 10^{\text{-1}}\) & \(5.35\times 10^{\text{-3}}\) & \(9.5\times 10^{\text{-2}}\) \\ 
\(d \bar{d} \rightarrow \tilde{g} \tilde{g}\) & \(4.942\times 10^2\) & \(4.35\times 10^{\text{-2}}\) & \(4.94\times 10^2\) & \(5.36\times 10^{\text{-2}}\) & \(3.06\times 10^{\text{-2}}\) \\ 
\(d \bar{d} \rightarrow g g\) & \(1.118\times 10^3\) & \(5.63\times 10^{\text{-2}}\) & \(1.117\times 10^3\) & \(5.8\times 10^{\text{-2}}\) & \(7.36\times 10^{\text{-2}}\) \\ 
\(\gamma \gamma \rightarrow \tilde{\chi}^+_1 \tilde{\chi}^-_1\) & \(3.398\times 10^1\) & \(4.79\times 10^{\text{-2}}\) & \(3.403\times 10^1\) & \(4.37\times 10^{\text{-2}}\) & \(-1.66\times 10^{\text{-1}}\) \\ 
\(\gamma \gamma \rightarrow W^- W^+\) & \(3.213\times 10^2\) & \(4.4\times 10^{\text{-2}}\) & \(3.211\times 10^2\) & \(6.91\times 10^{\text{-2}}\) & \(6.19\times 10^{\text{-2}}\) \\ 
\(\gamma \gamma \rightarrow \tilde{\chi}^+_2 \tilde{\chi}^-_2\) & \(3.695\times 10^1\) & \(4.71\times 10^{\text{-2}}\) & \(3.696\times 10^1\) & \(4.45\times 10^{\text{-2}}\) & \(-2.18\times 10^{\text{-2}}\) \\ 
\(\gamma \gamma \rightarrow d \bar{d}\) & \(1.21\) & \(7.26\times 10^{\text{-2}}\) & \(1.213\) & \(5.52\times 10^{\text{-2}}\) & \(-2.13\times 10^{\text{-1}}\) \\ 
\(\gamma \gamma \rightarrow t \bar{t}\) & \(2.013\times 10^1\) & \(4.89\times 10^{\text{-2}}\) & \(2.011\times 10^1\) & \(4.93\times 10^{\text{-2}}\) & \(1.02\times 10^{\text{-1}}\) \\ 
\(\gamma \gamma \rightarrow b \bar{b}\) & \(1.212\) & \(6.26\times 10^{\text{-2}}\) & \(1.215\) & \(9.1\times 10^{\text{-2}}\) & \(-2.47\times 10^{\text{-1}}\) \\ 
\(\gamma \gamma \rightarrow \tilde{t}_1 \tilde{t}_1^*\) & \(6.059\) & \(4.35\times 10^{\text{-2}}\) & \(6.065\) & \(6.72\times 10^{\text{-2}}\) & \(-1.04\times 10^{\text{-1}}\) \\ 
\(\gamma \gamma \rightarrow \tilde{t}_2 \tilde{t}_2^*\) & \(3.783\) & \(4.1\times 10^{\text{-2}}\) & \(3.772\) & \(4.39\times 10^{\text{-2}}\) & \(3.11\times 10^{\text{-1}}\) \\ 
\(\gamma \gamma \rightarrow \tilde{d}_1 \tilde{d}_1^*\) & \(2.434\times 10^{\text{-1}}\) & \(4.81\times 10^{\text{-2}}\) & \(2.437\times 10^{\text{-1}}\) & \(4.12\times 10^{\text{-2}}\) & \(-1.3\times 10^{\text{-1}}\) \\ 
\(\gamma \gamma \rightarrow \tilde{d}_2 \tilde{d}_2^*\) & \(2.572\times 10^{\text{-1}}\) & \(3.45\times 10^{\text{-2}}\) & \(2.57\times 10^{\text{-1}}\) & \(4.34\times 10^{\text{-2}}\) & \(8.89\times 10^{\text{-2}}\) \\ 
\(\gamma \gamma \rightarrow \tilde{e}_1 \tilde{e}_1^*\) & \(1.32\times 10^1\) & \(6.02\times 10^{\text{-2}}\) & \(1.318\times 10^1\) & \(5.18\times 10^{\text{-2}}\) & \(1.23\times 10^{\text{-1}}\) \\ 
\(\gamma \gamma \rightarrow \tilde{e}_2 \tilde{e}_2^*\) & \(1.392\times 10^1\) & \(5.19\times 10^{\text{-2}}\) & \(1.392\times 10^1\) & \(8.1\times 10^{\text{-2}}\) & \(-1.96\times 10^{\text{-2}}\) \\ 
\(\gamma \gamma \rightarrow \tilde{\tau}_1 \tilde{\tau}_1^*\) & \(1.405\times 10^1\) & \(4.13\times 10^{\text{-2}}\) & \(1.406\times 10^1\) & \(5.27\times 10^{\text{-2}}\) & \(-1.29\times 10^{\text{-1}}\) \\ 
\(\gamma \gamma \rightarrow \tilde{\tau}_2 \tilde{\tau}_2\) & \(1.312\times 10^1\) & \(8.15\times 10^{\text{-2}}\) & \(1.312\times 10^1\) & \(3.75\times 10^{\text{-2}}\) & \(-2.13\times 10^{\text{-2}}\) \\ 
\(\gamma \gamma \rightarrow H^- H^+\) & \(8.99\) & \(4.24\times 10^{\text{-2}}\) & \(8.983\) & \(4.38\times 10^{\text{-2}}\) & \(7.24\times 10^{\text{-2}}\) \\ 
\hline 
\end{longtable}

